Rendering Point Clouds with Compute Shaders and Vertex Order Optimization

While commodity GPUs provide a continuously growing range of features and sophisticated methods for accelerating compute jobs, many state-of-the-art solutions for point cloud rendering still rely on the provided point primitives (GL_POINTS, POINTLIST, ...) of graphics APIs for image synthesis. In this paper, we present several compute-based point cloud rendering approaches that outperform the hardware pipeline by up to an order of magnitude and achieve significantly better frame times than previous compute-based methods. Beyond basic closest-point rendering, we also introduce a fast, high-quality variant to reduce aliasing. We present and evaluate several variants of our proposed methods with different flavors of optimization, in order to ensure their applicability and achieve optimal performance on a range of platforms and architectures with varying support for novel GPU hardware features. During our experiments, the observed peak performance was reached rendering 796 million points (12.7GB) at rates of 62 to 64 frames per second (50 billion points per second, 802GB/s) on an RTX 3090 without the use of level-of-detail structures. We further introduce an optimized vertex order for point clouds to boost the efficiency of GL_POINTS by a factor of 5x in cases where hardware rendering is compulsory. We compare different orderings and show that Morton sorted buffers are faster for some viewpoints, while shuffled vertex buffers are faster in others. In contrast, combining both approaches by first sorting according to Morton-code and shuffling the resulting sequence in batches of 128 points leads to a vertex buffer layout with high rendering performance and low sensitivity to viewpoint changes.

==> chapters/pieces/perf_table.tex <==

% javascript:ace.edit($(".ace-editor-body")[0]).getSession().setUseWrapMode(false);


\begin{table*}[]
\begin{tabular*}{\textwidth}{@{}ll|rrrr|rr|r@{}}
\toprule
                                 &                           & \multicolumn{4}{c|}{\textbf{Basic}}                                                                                               & \multicolumn{2}{c|}{\textbf{High-Quality}}                   & \multicolumn{1}{c}{\textbf{Misc}} \\ \midrule
                                 & GPU \textbackslash Method & \multicolumn{1}{c}{atomicMin} & \multicolumn{1}{c}{early-z} & \multicolumn{1}{c}{ballot} & \multicolumn{1}{c|}{early-z \& ballot} & \multicolumn{1}{c}{hqs} & \multicolumn{1}{c|}{hqs (1x64bit)} & \multicolumn{1}{c}{just set}      \\ \midrule
\multirow{3}{*}{Heidentor (26M)} & 940MX                     & 1                             & 1                           & 1                          & 1                                      & 1                       & 1                                  & 1                                 \\
                                 & GTX 1060                  & 1                             & 1                           & 1                          & 1                                      & 1                       & 1                                  & 1                                 \\
                                 & RTX 3090                  & 1                             & 1                           & 1                          & 1                                      & 1                       & 1                                  & 1                                 \\
\multirow{3}{*}{Retz (145M)}     & 940MX                     & 1                             & 1                           & 1                          & 1                                      & 1                       & 1                                  & 1                                 \\
                                 & GTX 1060                  & 1                             & 1                           & 1                          & 1                                      & 1                       & 1                                  & 1                                 \\
                                 & RTX 3090                  & 1                             & 1                           & 1                          & 1                                      & 1                       & 1                                  & 1                                 \\
NVIDIA (500M)                    & RTX 3090                  & 1                             & 1                           & 1                          & 1                                      & 1                       & 1                                  & 1                                 \\
Niederweiden (1B)                & RTX 3090                  & 1                             & 1                           & 1                          & 1                                      & 1                       & 1                                  & 1                                 \\ \bottomrule
\end{tabular*}
\caption{Benchmarks with data sets in their original order. }
\label{tab:benchmarks}
\end{table*}

==> chapters/todos.tex <==

\section{TODOs}
\begin{itemize}
    \item Check all bibtex entries. Some are from google, and google often returns wrong entries, e.g., mixes authors and editors, etc. 
    \item Do not forget for discussion: 1060 dedup is slow, it has no support for partitioned instructions. On Turing is better, has support for match instruction. On Ampere should be better again, due to support for warp-wide reduce func.
\end{itemize}
